Lifshitz transition and magnetic superconductivity in flat band systems

A Lifshitz transition is a class of non-symmetry-breaking transitions typically associated with metallic systems wherein the Fermi surface changes its connectivity as the chemical potential sweeps through a band extremum or a saddle point. The phenomenology naturally adapts itself to the superconducting state, where the object that reconstructs is the manifold of minimum quasiparticle energy rather than the Fermi surface. This paper concerns Lifshitz-type transitions in multi-band superconductors. Thus, we focus on the attractive Hubbard--Kondo model on the two-dimensional Lieb lattice, with classical core spins coupled to the itinerant electrons, by laying recourse to a real-space Bogoliubov--de Gennes mean-field theory and an analytic Green's function calculation. The competition between the Kondo and pairing channels yields a magnetic superconductor throughout, with $(\pi,\pi)$ order near half filling giving way to $(0,\pi)$ and then, at stronger Kondo coupling, to an incommensurate spiral $(0,q)$. In such a multiband superconductor hosting a flat band, we identify two inequivalent Lifshitz-type transitions. With the core spins decoupled (the Kondo coupling set to zero), the minimum energy contour deforms with chemical potential, a hole pocket about $M$ opening into a perfectly nested square at $\mu=-2t$ and reconnecting into pockets about $\Gamma$; this nesting fixes where $(\pi,\pi)$ order sets in. At finite Kondo coupling, for certain chemical potential, the dimension of the manifold itself drops. We obtain it analytically for each magnetic order and show that only the spiral carries the minimum energy through zero, nucleating nodes and leaving a gapless magnetic superconductor, with clear signatures in the density of states and the spectral function.

==> prb_zero_modes_setup.tex <==
% INPUT THIS FILE ONCE IN THE PREAMBLE, before \begin{document}.
% No document class, page geometry, global font changes, or caption package.
% Intended for aps,prb,twocolumn in revtex4-1 and revtex4-2.
\RequirePackage{amsmath,amssymb,graphicx,longtable}
% Keep the BZ figure PDFs beside the manuscript for a flat arXiv upload.
% Momentum argument k+2q used throughout the appendix.
\providecommand{\kpq}{{\mathbf k+2\mathbf q}}
% Overlap matrices: identity, signed permutation, stripe, general.
\providecommand{\BZmatI}{\mathsf I}
\providecommand{\BZmatP}{\mathsf P}
\providecommand{\BZmatS}{\mathsf S}
\providecommand{\BZmatG}{\mathsf G}
% Fixed separate columns keep locus prose LEFT of the figure.
\providecommand{\BZfigure}[1]{\includegraphics[width=\linewidth]{#1.pdf}}
\providecommand{\BZrow}[6]{#1&#2&#3&#4&#5&\BZfigure{#6}}

